Quasi-static Soft Fixture Analysis of Rigid and Deformable Objects

We present a sampling-based approach to reasoning about the caging-based manipulation of rigid and a simplified class of deformable 3D objects subject to energy constraints. Towards this end, we propose the notion of soft fixtures extending earlier work on energy-bounded caging to include a broader set of energy function constraints and settings, such as gravitational and elastic potential energy of 3D deformable objects. Previous methods focused on establishing provably correct algorithms to compute lower bounds or analytically exact estimates of escape energy for a very restricted class of known objects with low-dimensional C-spaces, such as planar polygons. We instead propose a practical sampling-based approach that is applicable in higher-dimensional C-spaces but only produces a sequence of upper-bound estimates that, however, appear to converge rapidly to actual escape energy. We present 8 simulation experiments demonstrating the applicability of our approach to various complex quasi-static manipulation scenarios. Quantitative results indicate the effectiveness of our approach in providing upper-bound estimates for escape energy in quasi-static manipulation scenarios. Two real-world experiments also show that the computed normalized escape energy estimates appear to correlate strongly with the probability of escape of an object under randomized pose perturbation.

==> icra2024/tex/band-ear.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{sandybrown24416662}{RGB}{244,166,62}
\definecolor{seagreen4916384}{RGB}{49,163,84}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={# iterations},
xmajorgrids,
xmin=-2.15, xmax=45.15,
xtick style={color=black},
y grid style={darkgray176},
ylabel={potential energy / J},
ymajorgrids,
ymin=-0.0182201736993158, ymax=0.382623647685631,
ytick style={color=black}
]
\path [draw=sandybrown24416662, fill=sandybrown24416662, opacity=0.4]
(axis cs:0,0)
--(axis cs:0,0)
--(axis cs:1,0)
--(axis cs:2,0)
--(axis cs:3,0)
--(axis cs:4,0)
--(axis cs:5,0.0137389372326945)
--(axis cs:6,0.020433520439641)
--(axis cs:7,0.0315536793244082)
--(axis cs:8,0.0934668578469165)
--(axis cs:9,0.0907325846030632)
--(axis cs:10,0.0827693215900094)
--(axis cs:11,0.105906676612597)
--(axis cs:12,0.0997425408408701)
--(axis cs:13,0.123081128665719)
--(axis cs:14,0.0898872227121655)
--(axis cs:15,0.122497393210673)
--(axis cs:16,0.114181950260943)
--(axis cs:17,0.127719871929026)
--(axis cs:18,0.12849071263176)
--(axis cs:19,0.113252799948205)
--(axis cs:20,0.123201108758737)
--(axis cs:21,0.119179998083261)
--(axis cs:22,0.12531893531763)
--(axis cs:23,0.152720449248032)
--(axis cs:24,0.126663388014935)
--(axis cs:25,0.141603583239722)
--(axis cs:26,0.130898307627834)
--(axis cs:27,0.136860995662585)
--(axis cs:28,0.152152928849076)
--(axis cs:29,0.144364897618197)
--(axis cs:30,0.129419842811071)
--(axis cs:31,0.120033141599821)
--(axis cs:32,0.127489251877648)
--(axis cs:33,0.149711993251803)
--(axis cs:34,0.149584805106791)
--(axis cs:35,0.115315814189935)
--(axis cs:36,0.140945777218533)
--(axis cs:37,0.139574023450548)
--(axis cs:38,0.168568669522392)
--(axis cs:39,0.115593158082403)
--(axis cs:40,0.138304383288974)
--(axis cs:41,0.147031116387738)
--(axis cs:42,0.158425150643829)
--(axis cs:43,0.173272749480949)
--(axis cs:43,0.270337930797018)
--(axis cs:43,0.270337930797018)
--(axis cs:42,0.275459000233042)
--(axis cs:41,0.24126377864993)
--(axis cs:40,0.233158452759217)
--(axis cs:39,0.364403473986316)
--(axis cs:38,0.25737333953273)
--(axis cs:37,0.22574241786789)
--(axis cs:36,0.235798068400229)
--(axis cs:35,0.261052213337835)
--(axis cs:34,0.242592349287338)
--(axis cs:33,0.243121154418057)
--(axis cs:32,0.201762512831504)
--(axis cs:31,0.230644586271129)
--(axis cs:30,0.341368866004472)
--(axis cs:29,0.224459411455895)
--(axis cs:28,0.218820808848878)
--(axis cs:27,0.300882694802772)
--(axis cs:26,0.178864047639683)
--(axis cs:25,0.187107450123109)
--(axis cs:24,0.210383860139938)
--(axis cs:23,0.254064188210879)
--(axis cs:22,0.228658852934527)
--(axis cs:21,0.169677845258336)
--(axis cs:20,0.181822262402849)
--(axis cs:19,0.179968713122355)
--(axis cs:18,0.191521482465677)
--(axis cs:17,0.178037962704814)
--(axis cs:16,0.165361422127051)
--(axis cs:15,0.189518362769285)
--(axis cs:14,0.162712329868706)
--(axis cs:13,0.188954970813868)
--(axis cs:12,0.178093949517313)
--(axis cs:11,0.162207410113351)
--(axis cs:10,0.136766188604093)
--(axis cs:9,0.153044870173467)
--(axis cs:8,0.162780954595588)
--(axis cs:7,0.0915604638995122)
--(axis cs:6,0.0536329112211946)
--(axis cs:5,0.0501616890728072)
--(axis cs:4,0)
--(axis cs:3,0)
--(axis cs:2,0)
--(axis cs:1,0)
--(axis cs:0,0)
--cycle;

\addplot [thick, seagreen4916384]
table {%
0 0.0791429396691978
1 0.0807170309916805
2 0.0819958520719782
3 0.0838992590229207
4 0.0857455086178263
5 0.0876107878474174
6 0.0892069823134332
7 0.0874617811554714
8 0.0744161326361656
9 0.0651565470308488
10 0.0618602083212469
11 0.0580555865297608
12 0.0567025240219078
13 0.0560189881756921
14 0.0538904286194766
15 0.0522225789081798
16 0.0504266000542544
17 0.0488980881107534
18 0.0474679482713761
19 0.0463304556592927
20 0.0447881427850414
21 0.0429693934326145
22 0.0409731134137759
23 0.0391436127530323
24 0.0381446898944502
25 0.0367535078967213
26 0.0357186341135633
27 0.0356459367857118
28 0.0358289152059539
29 0.0358333298787113
30 0.0365674476823471
31 0.0372424573966696
32 0.0385009455053581
33 0.0402301160184437
34 0.0408349162165887
35 0.0407310251399294
36 0.039198025021421
37 0.0365727638113683
38 0.0330233190252093
39 0.0285584450897221
40 0.0239758729130939
41 0.0185217864352419
42 0.012681288336439
43 0.00989254466122671
};
\addlegendentry{total energy}
\addplot [thick, sandybrown24416662]
table {%
0 0
1 0
2 0
3 0
4 0
5 0.0109777730632016
6 0.0152340217292203
7 0.00860113543149858
8 0.0775124163455871
9 0.0742691109860152
10 0.0703119737211028
11 0.081614028728041
12 0.0766440621677084
13 0.115057552273845
14 0.0617481678926606
15 0.103220172980027
16 0.0944454349912032
17 0.118739047805405
18 0.100645221593911
19 0.101329958128781
20 0.118956380705054
21 0.098802065023669
22 0.108489718652847
23 0.143992672029599
24 0.107941133099467
25 0.126757866510516
26 0.117411541226235
27 0.142764129583304
28 0.125104189075686
29 0.11754187757466
30 0.129577496735139
31 0.0818620253347507
32 0.0908771031032801
33 0.117624866281802
34 0.112898142429796
35 0.104917752797433
36 0.0827890406386315
37 0.0999765085013195
38 0.150855438304125
39 0.131570902565136
40 0.0850750488756034
41 0.133089271437507
42 0.112430332851586
43 0.13917581264533
};
\addlegendentry{escape energy}
\end{axis}

\end{tikzpicture}


==> icra2024/tex/fish-shovel.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{sandybrown24416662}{RGB}{244,166,62}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={Escape energy in a dynamic scenario - ShovelFish},
x grid style={darkgray176},
xlabel={# iterations},
xmajorgrids,
xmin=-3.50017500875044, xmax=73.5036751837592,
xtick style={color=black},
y grid style={darkgray176},
ylabel={energy / J},
ymajorgrids,
ymin=-0.2, ymax=3.6,
ytick style={color=black}
]
\path [draw=sandybrown24416662, fill=sandybrown24416662, opacity=0.4]
(axis cs:0,0)
--(axis cs:0,0)
--(axis cs:1.13755687784389,1.03823386769232)
--(axis cs:2.27511375568778,1.39598528438367)
--(axis cs:3.41267063353168,0.877791737708901)
--(axis cs:4.55022751137557,0.959816736504835)
--(axis cs:5.68778438921946,1.05613892533137)
--(axis cs:6.82534126706335,0.864153071767281)
--(axis cs:7.96289814490725,1.05902093391642)
--(axis cs:9.10045502275114,0.421425081327182)
--(axis cs:10.238011900595,1.33333048045528)
--(axis cs:11.3755687784389,1.35244101752027)
--(axis cs:12.5131256562828,0.620373014703291)
--(axis cs:13.6506825341267,0.651513695405539)
--(axis cs:14.7882394119706,0.908071447863422)
--(axis cs:15.9257962898145,0.947661597166829)
--(axis cs:17.0633531676584,1.31963581606956)
--(axis cs:18.2009100455023,0.920451531077932)
--(axis cs:19.3384669233462,0.84398244882185)
--(axis cs:20.4760238011901,0.509360246315535)
--(axis cs:21.613580679034,0.867801033820097)
--(axis cs:22.7511375568778,0.904339826660183)
--(axis cs:23.8886944347217,1.17421007060075)
--(axis cs:25.0262513125656,0.54861514150086)
--(axis cs:26.1638081904095,1.04971418013112)
--(axis cs:27.3013650682534,0.900283759144947)
--(axis cs:28.4389219460973,0.251284116717893)
--(axis cs:29.5764788239412,0.759680652258656)
--(axis cs:30.7140357017851,0.953819685008166)
--(axis cs:31.851592579629,1.22481886108371)
--(axis cs:32.9891494574729,1.38825412076067)
--(axis cs:34.1267063353168,1.84989367131452)
--(axis cs:35.2642632131607,1.41435055693679)
--(axis cs:36.4018200910046,1.43758324931322)
--(axis cs:37.5393769688484,1.57970691102016)
--(axis cs:38.6769338466923,1.42799277775716)
--(axis cs:39.8144907245362,1.23187229903729)
--(axis cs:40.9520476023801,1.54124071402398)
--(axis cs:42.089604480224,1.45371410192215)
--(axis cs:43.2271613580679,1.65421532880323)
--(axis cs:44.3647182359118,1.69918488233666)
--(axis cs:45.5022751137557,1.65624141429496)
--(axis cs:46.6398319915996,0.910128875857797)
--(axis cs:47.7773888694435,0.675680229741845)
--(axis cs:48.9149457472874,-0.160718581718112)
--(axis cs:49.0024501225061,0)
--(axis cs:49.8774938746937,-0.114511804153429)
--(axis cs:50.7525376268813,-0.151545855848094)
--(axis cs:51.627581379069,0)
--(axis cs:52.5026251312566,0)
--(axis cs:53.3776688834442,-0.0021762392439075)
--(axis cs:54.2527126356318,-0.0739678561805089)
--(axis cs:55.1277563878194,0)
--(axis cs:56.002800140007,-0.14982386328065)
--(axis cs:56.8778438921946,-0.00167586874102439)
--(axis cs:57.7528876443822,-0.00355489040505396)
--(axis cs:58.6279313965698,-0.181418535353383)
--(axis cs:59.5029751487574,0)
--(axis cs:60.3780189009451,-0.0959019440148102)
--(axis cs:61.2530626531327,-0.127337319883415)
--(axis cs:62.1281064053203,-0.113272047984218)
--(axis cs:63.0031501575079,-0.207897629120442)
--(axis cs:63.8781939096955,-0.0596850410003882)
--(axis cs:64.7532376618831,0.478106027765717)
--(axis cs:65.6282814140707,0.638472023045862)
--(axis cs:66.5033251662583,1.41652292403708)
--(axis cs:67.3783689184459,1.32559064450562)
--(axis cs:68.2534126706335,1.25712478080384)
--(axis cs:69.1284564228211,0.542202066268613)
--(axis cs:70.0035001750088,1.71346840175277)
--(axis cs:70.0035001750088,3.7188249265225)
--(axis cs:70.0035001750088,3.7188249265225)
--(axis cs:69.1284564228211,2.86485458208415)
--(axis cs:68.2534126706335,3.07839920713433)
--(axis cs:67.3783689184459,2.67793875743735)
--(axis cs:66.5033251662583,3.24750457654806)
--(axis cs:65.6282814140707,3.0100343028104)
--(axis cs:64.7532376618831,2.313262334369)
--(axis cs:63.8781939096955,1.33330637433691)
--(axis cs:63.0031501575079,0.908733401326761)
--(axis cs:62.1281064053203,0.952042822222398)
--(axis cs:61.2530626531327,0.854189897959494)
--(axis cs:60.3780189009451,0.765861530786107)
--(axis cs:59.5029751487574,0)
--(axis cs:58.6279313965698,0.565333538034773)
--(axis cs:57.7528876443822,0.00662391601494445)
--(axis cs:56.8778438921946,0.0031226880516019)
--(axis cs:56.002800140007,0.279170543765463)
--(axis cs:55.1277563878194,0)
--(axis cs:54.2527126356318,0.137826152516154)
--(axis cs:53.3776688834442,0.00405504089790658)
--(axis cs:52.5026251312566,0)
--(axis cs:51.627581379069,0)
--(axis cs:50.7525376268813,0.456082574748656)
--(axis cs:49.8774938746937,0.473699473978519)
--(axis cs:49.0024501225061,0)
--(axis cs:48.9149457472874,0.520086597270931)
--(axis cs:47.7773888694435,2.08111952629304)
--(axis cs:46.6398319915996,2.53830413802223)
--(axis cs:45.5022751137557,2.75098009720459)
--(axis cs:44.3647182359118,3.08272225305486)
--(axis cs:43.2271613580679,2.94421561522182)
--(axis cs:42.089604480224,2.75666257371757)
--(axis cs:40.9520476023801,3.04505550229309)
--(axis cs:39.8144907245362,2.54410508516196)
--(axis cs:38.6769338466923,2.59101682229736)
--(axis cs:37.5393769688484,2.8258452769329)
--(axis cs:36.4018200910046,2.70489095614315)
--(axis cs:35.2642632131607,2.71906580327554)
--(axis cs:34.1267063353168,2.84371293007826)
--(axis cs:32.9891494574729,2.90168307788075)
--(axis cs:31.851592579629,2.60324707018411)
--(axis cs:30.7140357017851,2.40024777691663)
--(axis cs:29.5764788239412,1.97193893781591)
--(axis cs:28.4389219460973,1.52493516243522)
--(axis cs:27.3013650682534,2.04004271373263)
--(axis cs:26.1638081904095,2.08284467934622)
--(axis cs:25.0262513125656,1.51411147811519)
--(axis cs:23.8886944347217,2.22585351390888)
--(axis cs:22.7511375568778,2.15028264964033)
--(axis cs:21.613580679034,1.94995041500253)
--(axis cs:20.4760238011901,1.96920599652563)
--(axis cs:19.3384669233462,2.16896831339511)
--(axis cs:18.2009100455023,2.3652243224755)
--(axis cs:17.0633531676584,2.52046028639598)
--(axis cs:15.9257962898145,2.44680275019142)
--(axis cs:14.7882394119706,2.03716546339831)
--(axis cs:13.6506825341267,1.71818949494806)
--(axis cs:12.5131256562828,2.24590280519261)
--(axis cs:11.3755687784389,2.4015205427758)
--(axis cs:10.238011900595,2.00117492448616)
--(axis cs:9.10045502275114,2.54751899837534)
--(axis cs:7.96289814490725,1.9170742420101)
--(axis cs:6.82534126706335,2.23584602659115)
--(axis cs:5.68778438921946,1.65071551336737)
--(axis cs:4.55022751137557,2.14641759039566)
--(axis cs:3.41267063353168,1.84904039617877)
--(axis cs:2.27511375568778,1.93188440026696)
--(axis cs:1.13755687784389,2.20124234267544)
--(axis cs:0,0)
--cycle;

\addplot [thick, sandybrown24416662]
table {%
0 0
1.13755687784389 1.61973810518388
2.27511375568778 1.66393484232531
3.41267063353168 1.36341606694384
4.55022751137557 1.55311716345024
5.68778438921946 1.35342721934937
6.82534126706335 1.54999954917922
7.96289814490725 1.48804758796326
9.10045502275114 1.48447203985126
10.238011900595 1.66725270247072
11.3755687784389 1.87698078014804
12.5131256562828 1.43313790994795
13.6506825341267 1.1848515951768
14.7882394119706 1.47261845563087
15.9257962898145 1.69723217367912
17.0633531676584 1.92004805123277
18.2009100455023 1.64283792677672
19.3384669233462 1.50647538110848
20.4760238011901 1.23928312142058
21.613580679034 1.40887572441131
22.7511375568778 1.52731123815026
23.8886944347217 1.70003179225481
25.0262513125656 1.03136330980803
26.1638081904095 1.56627942973867
27.3013650682534 1.47016323643879
28.4389219460973 0.888109639576557
29.5764788239412 1.36580979503728
30.7140357017851 1.6770337309624
31.851592579629 1.91403296563391
32.9891494574729 2.14496859932071
34.1267063353168 2.34680330069639
35.2642632131607 2.06670818010617
36.4018200910046 2.07123710272818
37.5393769688484 2.20277609397653
38.6769338466923 2.00950480002726
39.8144907245362 1.88798869209963
40.9520476023801 2.29314810815854
42.089604480224 2.10518833781986
43.2271613580679 2.29921547201252
44.3647182359118 2.39095356769576
45.5022751137557 2.20361075574977
46.6398319915996 1.72421650694001
47.7773888694435 1.37839987801744
48.9149457472874 0.179684007776409
49.0024501225061 0
49.8774938746937 0.179593834912545
50.7525376268813 0.152268359450281
51.627581379069 0
52.5026251312566 0
53.3776688834442 0.000939400826999541
54.2527126356318 0.0319291481678228
55.1277563878194 0
56.002800140007 0.064673340242407
56.8778438921946 0.000723409655288757
57.7528876443822 0.00153451280494525
58.6279313965698 0.191957501340695
59.5029751487574 0
60.3780189009451 0.334979793385648
61.2530626531327 0.36342628903804
62.1281064053203 0.41938538711909
63.0031501575079 0.35041788610316
63.8781939096955 0.636810666668259
64.7532376618831 1.39568418106736
65.6282814140707 1.82425316292813
66.5033251662583 2.33201375029257
67.3783689184459 2.00176470097148
68.2534126706335 2.16776199396909
69.1284564228211 1.70352832417638
70.0035001750088 2.71614666413763
};
\addlegendentry{escape energy}
\end{axis}

\end{tikzpicture}


==> icra2024/tex/handbag-gripper.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{sandybrown24416662}{RGB}{244,166,62}
\definecolor{seagreen4916384}{RGB}{49,163,84}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
title={Escape energy in a dynamic scenario - HandbagGripper},
x grid style={darkgray176},
xlabel={# iterations},
xmajorgrids,
xmin=-1.75, xmax=36.75,
xtick style={color=black},
y grid style={darkgray176},
ylabel={potential energy / J},
ymajorgrids,
ymin=-0.0640114556040389, ymax=0.631619593124002,
ytick style={color=black}
]
\path [draw=sandybrown24416662, fill=sandybrown24416662, opacity=0.4]
(axis cs:0,0.153069523374678)
--(axis cs:0,0.0450388225254484)
--(axis cs:1,-0.032391862480037)
--(axis cs:2,0.0529341334745839)
--(axis cs:3,0.0515322012608259)
--(axis cs:4,0.0791416874234785)
--(axis cs:5,0.0614926393292477)
--(axis cs:6,0.0547794320525662)
--(axis cs:7,0.0870986222145275)
--(axis cs:8,0.154464216386126)
--(axis cs:9,0.110727219405756)
--(axis cs:10,0.141118571634264)
--(axis cs:11,0.197794154204955)
--(axis cs:12,0.194204204611021)
--(axis cs:13,0.112149435128658)
--(axis cs:14,0.239210965325578)
--(axis cs:15,0.239232331319523)
--(axis cs:16,0.236891023416399)
--(axis cs:17,0.252933119959053)
--(axis cs:18,0.227864823087558)
--(axis cs:19,0.258965887582398)
--(axis cs:20,0.252034999985829)
--(axis cs:21,0.169302138391374)
--(axis cs:22,0.215078356950258)
--(axis cs:23,0.254516128901229)
--(axis cs:24,0.280442523586785)
--(axis cs:25,0.272368213993833)
--(axis cs:26,0.262887241202097)
--(axis cs:27,0.297231741336797)
--(axis cs:28,0.339860980141217)
--(axis cs:29,0.240449921177316)
--(axis cs:30,0.200841104536265)
--(axis cs:31,0.246049639013212)
--(axis cs:32,0.277424786637398)
--(axis cs:33,0.257491155239079)
--(axis cs:34,0.246254292403835)
--(axis cs:35,0.260379682020163)
--(axis cs:35,0.397106220146587)
--(axis cs:35,0.397106220146587)
--(axis cs:34,0.466654423260118)
--(axis cs:33,0.489174538262215)
--(axis cs:32,0.472109441031568)
--(axis cs:31,0.430948680546845)
--(axis cs:30,0.57346327140991)
--(axis cs:29,0.438736107315501)
--(axis cs:28,0.423031335382907)
--(axis cs:27,0.525296972794916)
--(axis cs:26,0.40083083552382)
--(axis cs:25,0.469620625420257)
--(axis cs:24,0.458404796420011)
--(axis cs:23,0.428960562413075)
--(axis cs:22,0.400020033621521)
--(axis cs:21,0.487998462055546)
--(axis cs:20,0.465025682177335)
--(axis cs:19,0.4532638354756)
--(axis cs:18,0.468563018256757)
--(axis cs:17,0.462382985000168)
--(axis cs:16,0.407503365452841)
--(axis cs:15,0.50779485224937)
--(axis cs:14,0.49927201442819)
--(axis cs:13,0.455311102420047)
--(axis cs:12,0.452691682412774)
--(axis cs:11,0.440071151611275)
--(axis cs:10,0.450176305423801)
--(axis cs:9,0.379474300147906)
--(axis cs:8,0.447935317023319)
--(axis cs:7,0.380374792974917)
--(axis cs:6,0.260983515966725)
--(axis cs:5,0.24238424899524)
--(axis cs:4,0.366603529626361)
--(axis cs:3,0.331608659259126)
--(axis cs:2,0.196948873570519)
--(axis cs:1,0.350149760273854)
--(axis cs:0,0.153069523374678)
--cycle;

\addplot [thick, seagreen4916384]
table {%
0 0.32
1 0.328
2 0.336
3 0.344
4 0.352
5 0.36
6 0.368
7 0.376
8 0.384
9 0.392
10 0.4
11 0.408
12 0.416
13 0.424
14 0.432
15 0.44
16 0.448
17 0.456
18 0.464
19 0.472
20 0.48
21 0.488
22 0.496
23 0.504
24 0.512
25 0.52
26 0.528
27 0.536
28 0.544
29 0.552
30 0.56
31 0.568
32 0.576
33 0.584
34 0.592
35 0.6
};
\addlegendentry{total energy}
\addplot [thick, sandybrown24416662]
table {%
0 0.0491256349425061
1 0.0541523387042442
2 0.0673202264666783
3 0.0612463328981692
4 0.0749481405792984
5 0.063069265358189
6 0.072092708707967
7 0.0774722463347554
8 0.0760670274672013
9 0.0854261008143503
10 0.109524965430245
11 0.167235435708735
12 0.0897559710073874
13 0.113894858982453
14 0.182590761498666
15 0.131913502883173
16 0.163133533317564
17 0.139281784308602
18 0.101775529007965
19 0.154245108140268
20 0.167722680393827
21 0.159951775408222
22 0.183756836499947
23 0.186970160093456
24 0.19641209448371
25 0.19108779428897
26 0.221527810931485
27 0.328422544656747
28 0.311603237285216
29 0.193482514846382
30 0.198989179775745
31 0.212132173508059
32 0.260895773535073
33 0.233907923677604
34 0.188308002495534
35 0.236420025050796
};
\addlegendentry{escape energy}
\end{axis}

\end{tikzpicture}


==> icra2024/tex/phys-experiment/test.tex <==
\begin{tikzpicture}[
  blacknode/.style={shape=circle, draw=black, line width=2},
  bluenode/.style={shape=rectangle, draw=blue, line width=2},
  greennode/.style={shape=circle, draw=green, line width=2},
  rednode/.style={shape=circle, draw=red, line width=2}
]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{sandybrown24416662}{RGB}{244,166,62}
\definecolor{seagreen4916384}{RGB}{49,163,84}
\definecolor{slateblue117107177}{RGB}{117,107,177}
\definecolor{steelblue43140190}{RGB}{43,140,190}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Escape Depth (dm)},
xmin=0.03, xmax=0.58,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Perturbation Level},
ymin=0.3, ymax=0.92,
ytick style={color=black}
]


\draw (0.3, 0.6) node[draw, shape=rectangle, minimum size=1mm] {};
\draw (0.2, 0.6) node[draw, shape=circle, minimum size=1mm] {};
\draw (0.3, 0.7) node[draw, shape=regular polygon, regular polygon sides=3, minimum size=1mm] {};
\draw (.1, .4) node[star, draw, minimum size=1mm] {};

% \node[regular polygon,regular polygon sides=3, draw, shape border rotate=180] at (0,0){Non-rotated text};
% \node[isosceles triangle,
%     draw,
%     fill=cyan!30,
%     minimum size =3cm] (T)at (0,0){};
    
\matrix [draw,below left] at (0.2,0.9) {
  \node [blacknode,label=right:Foo] {}; \\
  \node [bluenode,label=right:Bar] {}; \\
  \node [greennode,label=right:Baz] {}; \\
  \node [rednode,label=right:Foobar] {}; \\
};

\end{axis}

\end{tikzpicture}


==> icra2024/tex/quantitative-tests/test01/test01-3basic.tex <==
% This file was created with tikzplotlib v0.10.1.
% \begin{tikzpicture}[font=\footnotesize]

% \definecolor{darkgray176}{RGB}{176,176,176}
% \definecolor{lightgray204}{RGB}{204,204,204}
% \definecolor{orangered2405932}{RGB}{240,59,32}
% \definecolor{seagreen4916384}{RGB}{49,163,84}
% \definecolor{slateblue117107177}{RGB}{117,107,177}
% \definecolor{steelblue43140190}{RGB}{43,140,190}
% \definecolor{sandybrown24416662}{RGB}{244,166,62}

\begin{axis}[name=one,
width=0.2\linewidth, height=0.22\linewidth, scale only axis,
at={($(zero.east)+(.05\linewidth,-.098\linewidth)$)},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=inside,
tick pos=left,
x grid style={darkgray176},
x label style={at={(axis description cs:0.5,-0.05)}, anchor=north},
xlabel={frame},
% xmajorgrids,
xmin=-0.02, xmax=26,
xtick style={color=black},
y grid style={darkgray176},
y label style={at={(axis description cs:-0.105,.5)},anchor=south},
ylabel={escape energy / J},
% ymajorgrids,
ymin=0.40380220842007, ymax=0.964330563693418,
ytick style={color=black}
]
\path [draw=seagreen4916384, fill=seagreen4916384, opacity=0.3]
(axis cs:0,0.525946507517135)
--(axis cs:0,0.500259125798675)
--(axis cs:1,0.466144766465083)
--(axis cs:2,0.442777049052475)
--(axis cs:3,0.437464532415399)
--(axis cs:4,0.450662879531412)
--(axis cs:5,0.458801688875334)
--(axis cs:6,0.451955411626336)
--(axis cs:7,0.466800710941389)
--(axis cs:8,0.470316872456195)
--(axis cs:9,0.498194123617186)
--(axis cs:10,0.511105101313737)
--(axis cs:11,0.547850764531378)
--(axis cs:12,0.567842725939452)
--(axis cs:13,0.628696496344851)
--(axis cs:14,0.646900836527651)
--(axis cs:15,0.698813717846339)
--(axis cs:16,0.731192142175168)
--(axis cs:17,0.776712527585807)
--(axis cs:18,0.80646251513801)
--(axis cs:19,0.829405991697748)
--(axis cs:20,0.839502997033981)
--(axis cs:21,0.847761996249204)
--(axis cs:22,0.849597302062426)
--(axis cs:23,0.883101724971631)
--(axis cs:24,0.876774824570442)
--(axis cs:25,0.897174590816215)
--(axis cs:26,0.896351201788614)
--(axis cs:26,0.935867739450683)
--(axis cs:26,0.935867739450683)
--(axis cs:25,0.924009154472332)
--(axis cs:24,0.910629641439055)
--(axis cs:23,0.909053697193435)
--(axis cs:22,0.869831391394339)
--(axis cs:21,0.85778343451517)
--(axis cs:20,0.869817909395439)
--(axis cs:19,0.863321044790904)
--(axis cs:18,0.837855735344659)
--(axis cs:17,0.809240425256959)
--(axis cs:16,0.751163222555769)
--(axis cs:15,0.719942452257698)
--(axis cs:14,0.681235041698607)
--(axis cs:13,0.63910137428189)
--(axis cs:12,0.587380226769237)
--(axis cs:11,0.572278585340605)
--(axis cs:10,0.553558292662113)
--(axis cs:9,0.521796109354216)
--(axis cs:8,0.505251554446467)
--(axis cs:7,0.509635994004979)
--(axis cs:6,0.486342058343626)
--(axis cs:5,0.489934191868603)
--(axis cs:4,0.474889558792541)
--(axis cs:3,0.464956759578798)
--(axis cs:2,0.471370573724698)
--(axis cs:1,0.483537213162297)
--(axis cs:0,0.525946507517135)
--cycle;

\path [draw=slateblue117107177, fill=slateblue117107177, opacity=0.3]
(axis cs:0,0.521050050631555)
--(axis cs:0,0.499578959590191)
--(axis cs:1,0.480203150454718)
--(axis cs:2,0.457603836589974)
--(axis cs:3,0.455736003586645)
--(axis cs:4,0.461303384876437)
--(axis cs:5,0.46617081117821)
--(axis cs:6,0.465054409003149)
--(axis cs:7,0.481826802685142)
--(axis cs:8,0.50281947107925)
--(axis cs:9,0.500149798187073)
--(axis cs:10,0.545349903365428)
--(axis cs:11,0.550556668621688)
--(axis cs:12,0.582211541286494)
--(axis cs:13,0.616491198515665)
--(axis cs:14,0.667559356222836)
--(axis cs:15,0.703813891456953)
--(axis cs:16,0.732175948819523)
--(axis cs:17,0.781724779211874)
--(axis cs:18,0.835932689007293)
--(axis cs:19,0.824557227612323)
--(axis cs:20,0.842660105414051)
--(axis cs:21,0.859474311409451)
--(axis cs:22,0.868341539785369)
--(axis cs:23,0.86736210412199)
--(axis cs:24,0.881995553977585)
--(axis cs:25,0.894226204376771)
--(axis cs:26,0.908226676246851)
--(axis cs:26,0.938852002090084)
--(axis cs:26,0.938852002090084)
--(axis cs:25,0.907337421772445)
--(axis cs:24,0.889122489639808)
--(axis cs:23,0.89091000890825)
--(axis cs:22,0.885845155021004)
--(axis cs:21,0.86833195408343)
--(axis cs:20,0.872333743498055)
--(axis cs:19,0.852574818500154)
--(axis cs:18,0.847606054938181)
--(axis cs:17,0.806611376373538)
--(axis cs:16,0.751811777866098)
--(axis cs:15,0.731863754384718)
--(axis cs:14,0.678372055251278)
--(axis cs:13,0.64114656620954)
--(axis cs:12,0.597363261299673)
--(axis cs:11,0.58314254711499)
--(axis cs:10,0.568074414038258)
--(axis cs:9,0.516841218574987)
--(axis cs:8,0.516607450163957)
--(axis cs:7,0.493982637401375)
--(axis cs:6,0.481135578349397)
--(axis cs:5,0.485687382684174)
--(axis cs:4,0.47395768338624)
--(axis cs:3,0.471839325122807)
--(axis cs:2,0.481290789947278)
--(axis cs:1,0.498173274621465)
--(axis cs:0,0.521050050631555)
--cycle;

\path [draw=steelblue43140190, fill=steelblue43140190, opacity=0.3]
(axis cs:0,0.513522811223044)
--(axis cs:0,0.508037657132502)
--(axis cs:1,0.474519811297825)
--(axis cs:2,0.454018094458947)
--(axis cs:3,0.453188438761243)
--(axis cs:4,0.44303257656914)
--(axis cs:5,0.454630590302902)
--(axis cs:6,0.449325463112082)
--(axis cs:7,0.462578671598202)
--(axis cs:8,0.489631638842277)
--(axis cs:9,0.495427063120323)
--(axis cs:10,0.52391376009165)
--(axis cs:11,0.563382128733005)
--(axis cs:12,0.587798458558286)
--(axis cs:13,0.616120711250072)
--(axis cs:14,0.649944925159442)
--(axis cs:15,0.695463219204088)
--(axis cs:16,0.748812446312593)
--(axis cs:17,0.779294128759806)
--(axis cs:18,0.823136585903427)
--(axis cs:19,0.834604437865514)
--(axis cs:20,0.841978645132384)
--(axis cs:21,0.847774337067022)
--(axis cs:22,0.861837878931598)
--(axis cs:23,0.877607159032678)
--(axis cs:24,0.879974975322623)
--(axis cs:25,0.892176871475517)
--(axis cs:26,0.907623865648641)
--(axis cs:26,0.915596014554598)
--(axis cs:26,0.915596014554598)
--(axis cs:25,0.923419816644459)
--(axis cs:24,0.893782695753892)
--(axis cs:23,0.891485610539571)
--(axis cs:22,0.884541931095842)
--(axis cs:21,0.852729413541629)
--(axis cs:20,0.860707442625467)
--(axis cs:19,0.852276925076519)
--(axis cs:18,0.826283920415775)
--(axis cs:17,0.784909603393082)
--(axis cs:16,0.751903342324537)
--(axis cs:15,0.703430811008733)
--(axis cs:14,0.662768994518735)
--(axis cs:13,0.619508104608658)
--(axis cs:12,0.590601225885893)
--(axis cs:11,0.580745265629529)
--(axis cs:10,0.536415787531916)
--(axis cs:9,0.506797224411817)
--(axis cs:8,0.501469728149118)
--(axis cs:7,0.471400817968687)
--(axis cs:6,0.468886929066653)
--(axis cs:5,0.460707534886823)
--(axis cs:4,0.459881280988876)
--(axis cs:3,0.458004324152171)
--(axis cs:2,0.466641240303488)
--(axis cs:1,0.49666605982206)
--(axis cs:0,0.513522811223044)
--cycle;

\addplot [thick, seagreen4916384]
table {%
0 0.513102816657905
1 0.47484098981369
2 0.457073811388586
3 0.451210645997099
4 0.462776219161977
5 0.474367940371969
6 0.469148734984981
7 0.488218352473184
8 0.487784213451331
9 0.509995116485701
10 0.532331696987925
11 0.560064674935991
12 0.577611476354344
13 0.633898935313371
14 0.664067939113129
15 0.709378085052019
16 0.741177682365468
17 0.792976476421383
18 0.822159125241334
19 0.846363518244326
20 0.85466045321471
21 0.852772715382187
22 0.859714346728383
23 0.896077711082533
24 0.893702233004749
25 0.910591872644274
26 0.916109470619648
};
\addlegendentry{bi.}
\addplot [thick, slateblue117107177]
table {%
0 0.510314505110873
1 0.489188212538091
2 0.469447313268626
3 0.463787664354726
4 0.467630534131339
5 0.475929096931192
6 0.473094993676273
7 0.487904720043258
8 0.509713460621603
9 0.50849550838103
10 0.556712158701843
11 0.566849607868339
12 0.589787401293084
13 0.628818882362603
14 0.672965705737057
15 0.717838822920835
16 0.74199386334281
17 0.794168077792706
18 0.841769371972737
19 0.838566023056238
20 0.857496924456053
21 0.863903132746441
22 0.877093347403187
23 0.87913605651512
24 0.885559021808696
25 0.900781813074608
26 0.923539339168467
};
\addlegendentry{cons.}
\addplot [thick, steelblue43140190]
table {%
0 0.510780234177773
1 0.485592935559942
2 0.460329667381218
3 0.455596381456707
4 0.451456928779008
5 0.457669062594862
6 0.459106196089368
7 0.466989744783445
8 0.495550683495698
9 0.50111214376607
10 0.530164773811783
11 0.572063697181267
12 0.58919984222209
13 0.617814407929365
14 0.656356959839088
15 0.699447015106411
16 0.750357894318565
17 0.782101866076444
18 0.824710253159601
19 0.843440681471017
20 0.851343043878925
21 0.850251875304325
22 0.87318990501372
23 0.884546384786124
24 0.886878835538258
25 0.907798344059988
26 0.911609940101619
};
\addlegendentry{BIT*}
\addplot [thick, orangered2405932]
table {%
0 0.488486548660846
1 0.458012356665786
2 0.437614458014676
3 0.429280770023404
4 0.431359400450557
5 0.436192327347097
6 0.440941453289702
7 0.452210203610543
8 0.466816808795636
9 0.485220884491298
10 0.507641193555092
11 0.534656583591843
12 0.565798715160739
13 0.600407836132002
14 0.637687911224281
15 0.676761122737124
16 0.716675741041223
17 0.756406363424851
18 0.794883639493274
19 0.816094182463832
20 0.823526014238891
21 0.832085381610828
22 0.841440878620931
23 0.852052279116178
24 0.864953264140803
25 0.879599163272006
26 0.898601858649581
};
\addlegendentry{ref.}

\addplot [black, dashed, forget plot]
table {%
4.0 0.1
4.0 1
};
\draw (axis cs:4,0.42) node[
  scale=0.9,
  anchor=base west,
  text=black,
  rotate=0.0
]{A};

\addplot [black, dashed, forget plot]
table {%
13.0 0.1
13.0 1
};
\draw (axis cs:13,0.42) node[
  scale=0.9,
  anchor=base west,
  text=black,
  rotate=0.0
]{B};

\addplot [black, dashed, forget plot]
table {%
21.0 0.1
21.0 1
};
\draw (axis cs:21,0.42) node[
  scale=0.9,
  anchor=base west,
  text=black,
  rotate=0.0
]{C};

\draw (axis cs:22,0.5) node[
  scale=1,
  anchor=base west,
  text=red,
  rotate=0.0
]{(ii)};
\end{axis}

% \end{tikzpicture}


==> icra2024/tex/quantitative-tests/test04/test04.tex <==
% This file was created with tikzplotlib v0.10.1.
% % \begin{tikzpicture}[font=\footnotesize]

% % \definecolor{darkgray176}{RGB}{176,176,176}
% % \definecolor{lightgray204}{RGB}{204,204,204}
% % \definecolor{seagreen4916384}{RGB}{49,163,84}
% % \definecolor{slateblue117107177}{RGB}{117,107,177}
% % \definecolor{steelblue43140190}{RGB}{43,140,190}

\begin{axis}[name=three,
width=0.2\linewidth, height=0.22\linewidth, scale only axis,
at={($(two.east)+(.05\linewidth,-.11\linewidth)$)},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=inside,
tick pos=left,
x grid style={darkgray176},
x label style={at={(axis description cs:0.5,-0.05)}, anchor=north},
xlabel={\# control points},
xmin=3, xmax=9,
xtick style={color=black},
y label style={at={(axis description cs:-0.105,.5)},anchor=south},
y grid style={darkgray176},
ylabel={escape energy / J},
ymin=0.05, ymax=0.7,
ytick style={color=black}
]
\path [draw=steelblue43140190, fill=slateblue117107177, opacity=0.3]
(axis cs:3,0.247877286820441)
--(axis cs:3,0.226957941536287)
--(axis cs:4,0.170210554870321)
--(axis cs:5,0.175192545565182)
--(axis cs:6,0.211742575264267)
--(axis cs:7,0.291748083403441)
--(axis cs:8,0.334004710803269)
--(axis cs:9,0.461745373709534)
--(axis cs:9,0.65889211151978)
--(axis cs:9,0.65889211151978)
--(axis cs:8,0.404059673343059)
--(axis cs:7,0.353023946044547)
--(axis cs:6,0.259174661652487)
--(axis cs:5,0.211877073994421)
--(axis cs:4,0.190948518747258)
--(axis cs:3,0.247877286820441)
--cycle;


\addplot [thick, seagreen4916384, mark=asterisk, mark size=3, mark options={solid}]
table {%
3 1
4 1
5 1
6 1
7 1
8 1
9 1
};
\addlegendentry{dimension}

\addplot [thick, steelblue43140190, mark=*, mark size=2, mark options={solid}]
table {%
3 0.237417614178364
4 0.18057953680879
5 0.193534809779802
6 0.235458618458377
7 0.322386014723994
8 0.369032192073164
9 0.560318742614657
};
\addlegendentry{BIT*}

\addplot [thick, orangered2405932, mark=*, mark size=2, mark options={solid}]
table {%
3 0.20557206
4 0.12182048
5 0.100476017713583
6 0.09136536
7 0.0865214089075129
8 0.083604360073597
9 0.0816990636286701
};
\addlegendentry{ref.}

\draw (axis cs:8,0.15) node[
  scale=1,
  anchor=base west,
  text=red,
  rotate=0.0
]{(iv)};

\end{axis}

\begin{axis}[name=one,
width=0.2\linewidth, height=0.22\linewidth, scale only axis,
% at=(two.east), anchor={(-.055\linewidth,.11\linewidth)},
at={($(two.east)+(.05\linewidth,-.11\linewidth)$)},
% at={($(two.east)+(-.055\linewidth,.11\linewidth)$)},
axis y line=right,
tick align=inside,
x grid style={darkgray176},
xmin=3, xmax=9,
xtick pos=left,
xtick style={color=black},
y grid style={darkgray176},
y label style={at={(axis description cs:1.18,.5)},anchor=south},
ylabel={dim},
ymin=6.4, ymax=19.6,
ytick pos=right,
ytick style={color=black},
yticklabel style={anchor=west}
]
\addplot [thick, seagreen4916384, mark=asterisk, mark size=3, mark options={solid}]
table {%
3 7
4 9
5 11
6 13
7 15
8 17
9 19
};
\end{axis}






% \begin{axis}[name=two,
% width=0.4\linewidth, height=0.4\linewidth, scale only axis,
% % enlargelimits=false,
% at=(one.north east), anchor=north west,
% yticklabels={,,}, xticklabels={,,},
% % axis line style={draw=none},
% tick style={draw=none}
% ]
% \addplot graphics [includegraphics, xmin=0, xmax=1023.5, ymin=1023.5, ymax=0] {icra2024/figures/test04/band-hourglass.png};
% % \draw (axis cs:0,-0.1) node[
% %   scale=0.9,
% %   anchor=base west,
% %   text=black,
% %   rotate=0.0
% % ]{A};
% \end{axis}


% \end{tikzpicture}

